Spatially Disaggregated Energy Consumption and Emissions in End-use Sectors for Germany and Spain

High-resolution energy consumption and emissions datasets are essential for localized policy-making, resource optimization, and climate action planning. They enable municipalities to monitor mitigation strategies and foster engagement among governments, businesses, and communities. However, smaller municipalities often face data limitations that hinder tailored climate strategies. This study generates detailed final energy consumption and emissions data at the local administrative level for Germany and Spain. Using national datasets, we apply spatial disaggregation techniques with open data sources. A key innovation is the application of XGBoost for imputing missing data, combined with a stepwise spatial disaggregation process incorporating district- and province-level statistics. Prioritizing reproducibility, our open-data approach provides a scalable framework for municipalities to develop actionable climate plans. To ensure transparency, we assess the reliability of imputed values and assign confidence ratings to the disaggregated data.

==> tables/proxy_mapping_fec.tex <==
\begin{table}[ht]
    \centering
    % \begin{tabular}{|p{5cm}|p{8cm}|l|}
    \begin{NiceTabular}{p{4cm}p{5cm}p{5cm}}[hvlines]
    \hline
        &  \multicolumn{2}{|c|}{\textbf{LAU Proxy}}  \\
    \hline
    \multicolumn{1}{|c|}{\textbf{FEC source}} & \multicolumn{1}{c|}{\textbf{Germany}} & \multicolumn{1}{c|}{\textbf{Spain}} \\
    \hline
    Iron and steel industries & \multicolumn{2}{c|}{\cellcolor{red!25}Number of iron and steel industries} \\
    \hline
    Non-ferrous metals industries & \multicolumn{2}{c|}{\cellcolor{red!25}Number of non-ferrous metals industries} \\
    \hline
    Chemical and petrochemical industries & \multicolumn{2}{c|}{\cellcolor{red!25}Number of chemical industries + Number of refineries} \\
    \hline
    Non-metallic minerals industries & \multicolumn{2}{c|}{\cellcolor{red!25}Number of non-metallic minerals industries} \\
    \hline
    Mining and quarrying & \multicolumn{2}{c|}{\cellcolor{green!25}Mineral extraction sites cover} \\
    \hline
    Paper, pulp, and printing industries & \multicolumn{2}{c|}{\cellcolor{red!25}Number of paper and printing industries} \\
    \hline
    Wood and wood products industries & \cellcolor{green!25}Employment in wood processing & \cellcolor{blue!25}Employment in manufacturing \\
    \hline
    Transport equipment industries & \cellcolor{green!25}Employment in mechanical and automotive engineering &  \cellcolor{blue!25}Employment in manufacturing \\
    \hline
    Machinery industries & \cellcolor{green!25}Employment in mechatronics, energy and electrical &  \cellcolor{blue!25}Employment in manufacturing \\
    \hline
    Food, beverages, and tobacco industries & \cellcolor{green!25}Employment in food and beverage manufacturing &  \cellcolor{blue!25}Employment in manufacturing \\
    \hline
    Construction & \cellcolor{green!25}Employment in construction &  \cellcolor{blue!25}Employment in manufacturing \\
    \hline
    Textile and leather industries & \cellcolor{green!25}Employment in textile and leather manufacturing &  \cellcolor{blue!25}Employment in manufacturing \\
    \hline
    Rail transport & \multicolumn{2}{c|}{\cellcolor{green!25}Railway network} \\
    \hline
    Road transport & \cellcolor{green!25}(Road transport of freight) +
                                                    (3.83 * Number of passenger cars emission group euro 1) + 
                                                (1.78 * Number of passenger cars emission group euro 2) +
                                                (1.25 * Number of passenger cars emission group euro 3) +
                                                (0.825 * Number of passenger cars emission group euro 4) +
                                                (0.735 * Number of passenger cars emission group euro 5) +
                                                (0.6745 * Number of passenger cars emission group euro 6r) +
                                                (0.6745 * Number of passenger cars emission group euro 6dt) +
                                                (0.6745 * Number of passenger cars emission group euro 6d) +
                                                (3.83 * Number of passenger cars emission group euro other)
                                            
                                            &  \cellcolor{green!25}Road transport of freight + Average daily traffic - light duty vehicles  \\
    \hline
    Domestic aviation & \multicolumn{2}{c|}{\cellcolor{green!25}Air transport of freight + Air transport of passengers} \\    
    \hline
    Domestic navigation & \multicolumn{2}{c|}{\cellcolor{green!25}Port areas cover} \\    
    \hline
    Households & \cellcolor{green!25}Residential building living area * Heating degree days &  \cellcolor{blue!25}Number of dwellings * Heating degree days \\
    \hline
    Commerce & \cellcolor{green!25}Non-residential building living area * Heating degree days &  \cellcolor{blue!25}Number of commercial and service companies * Heating degree days \\
    \hline
    Agriculture and forestry & \multicolumn{2}{c|}{\cellcolor{green!25}Employment in agriculture, forestry, and fishing} \\
    \hline
\end{NiceTabular}
\caption{\label{tab:proxy_mapping_fec}The spatial proxies used to disaggregate each FEC data from NUTS0 to LAU level,
along with the assigned confidence level. Refer to Table \ref{tab:imputation_confidence_level} for confidence level color schema.}
\end{table}

